$P^2$GNN: Two Prototype Sets to boost GNN Performance

Message Passing Graph Neural Networks (MP-GNNs) have garnered attention for addressing various industry challenges, such as user recommendation and fraud detection. However, they face two major hurdles: (1) heavy reliance on local context, often lacking information about the global context or graph-level features, and (2) assumption of strong homophily among connected nodes, struggling with noisy local neighborhoods. To tackle these, we introduce $P^2$GNN, a plug-and-play technique leveraging prototypes to optimize message passing, enhancing the performance of the base GNN model. Our approach views the prototypes in two ways: (1) as universally accessible neighbors for all nodes, enriching global context, and (2) aligning messages to clustered prototypes, offering a denoising effect. We demonstrate the extensibility of our proposed method to all message-passing GNNs and conduct extensive experiments across 18 datasets, including proprietary e-commerce datasets and open-source datasets, on node recommendation and node classification tasks. Results show that $P^2$GNN outperforms production models in e-commerce and achieves the top average rank on open-source datasets, establishing it as a leading approach. Qualitative analysis supports the value of global context and noise mitigation in the local neighborhood in enhancing performance.

==> tables/tab_params_space.tex <==
%We list the grid search space for hyper-parameters as follows.
\begin{table}[H]
\caption{Hyperparameter search space on small-scale datasets}
\centering
\begin{tabular}{|c|c|}
    \hline
    {\bf Notation} & {\bf Range} \\ \hline
     lr  & $\{0.01, 0.005\}$ \\ \hline 
      dropout & $[0, 0.9]$ \\ \hline 
    %   early\_stopping  & $\{40, 200, 300\}$ \\ \hline 
        weight\_decay  & $\{1\mathrm{e}{-5}, 5\mathrm{e}{-5}, 1\mathrm{e}{-4}\}$ \\\hline 
        
        $K_\mathcal{N}$  & $\{2, 4, 8, 16, 32, 64, 128\}$ \\\hline 
        
        $K_\mathcal{A}$  & $\{2, 4, 8, 16, 32, 64, 128\}$ \\\hline 
        
        \lambda_a, \lambda_d, \lambda_s  &  $\{1\mathrm{e}{-4}, 1\mathrm{e}{-3}, 1\mathrm{e}{-2}, 1\mathrm{e}{-1}, 1, 10\}$ \\\hline 
        
        %  $\alpha$  & $[0,1]$ \\ \hline 
        %  $\beta_1$  & $\{0, 1, 10\}$ \\ \hline 
        %  $ \beta_2$  & $\{0.1, 1, 10, 10^2, 10^3\}$ \\ \hline  
        %   $\gamma$ & $[0, 0.9]$ \\ \hline 
            % norm\_layers  & $\{1, 2, 3\}$ \\ \hline 
            %  max\_hop\_count $K$  & $[1, 6]$ \\ \hline 
\end{tabular}
\label{table:grid_search_small}
%\end{small}
\end{table}


\begin{table}[H]
\caption{Hyper-parameter search space on large-scale datasets}
\centering
\begin{tabular}{|c|c|}
    \hline
    {\bf Notation} & {\bf Range} \\ \hline
     lr  & $\{0.01, 0.005, 0.001\}$ \\ \hline 
      dropout & $[0, 0.9]$ \\ \hline 
        weight\_decay  & $\{0, 1\mathrm{e}{-3}, 1\mathrm{e}{-2}, 1\mathrm{e}{-1}\}$ \\ \hline 
        $K_\mathcal{N}$  & $\{2, 4, 8, 16, 32, 64, 128\}$ \\\hline 
        
        $K_\mathcal{A}$  & $\{2, 4, 8, 16, 32, 64, 128\}$ \\\hline 
        
        \lambda_a, \lambda_d, \lambda_s  &  $\{1\mathrm{e}{-4}, 1\mathrm{e}{-3}, 1\mathrm{e}{-2}, 1\mathrm{e}{-1}, 1, 10\}$ \\\hline 
        %  $\alpha$  & $\{0.1, 0.5, 0.9\}$ \\ \hline 
        %  $\beta_1$  & $\{0, 0.1, 1\}$ \\ \hline 
        %  $ \beta_2$  & $\{0.1, 1\}$ \\ \hline  
        %   $\gamma$ & $\{0.1, 0.5, 0.9\}$ \\ \hline 
            % norm\_layers  & $\{1, 2, 3\}$ \\ \hline 
            %  max\_hop\_count $K$  & $\{1, 2, 3\}$ \\ \hline   
\end{tabular}
\label{table:grid_search_large}
%\end{small}
\end{table}
